EviDense: a Graph-based Method for Finding Unique High-impact Events with Succinct Keyword-based Descriptions

Despite the significant efforts made by the research community in recent years, automatically acquiring valuable information about high impact-events from social media remains challenging. We present EviDense, a graph-based approach for finding high-impact events (such as disaster events) in social media. One of the challenges we address in our work is to provide for each event a succinct keyword-based description, containing the most relevant information about it, such as what happened, the location, as well as its timeframe. We evaluate our approach on a large collection of tweets posted over a period of 19 months, using a crowdsourcing platform. Our evaluation shows that our method outperforms state-of-the-art approaches for the same problem, in terms of having higher precision, lower number of duplicates, and presenting a keyword-based description that is succinct and informative. We further improve the results of our algorithm by incorporating news from mainstream media. A preliminary version of this work was presented as a 4-pages short paper at ICWSM 2018.

==> casestudy.tex <==
\subsection{Beyond Crisis Events}

In this section, we study a different category of events in order to understand whether our approach can effectively be used to detect other classes of events. We focus on political events. In order to obtain tweets relevant to our task, we create a lexicon of terms related to politics. We include keywords like ''protest'', ''immigration'', ''election'' or ''government'', however, better results could be obtained if the list of words is produced in the same fashion as the crisis lexicon provided in~\cite{Olteanu2014}.
Detecting bursts in the mentions of locations turned out to be an effective method to detect crisis events. In the case of political events, politicians might play an important role in this kind of events. Therefore, we detect bursts in the mentions of locations or persons, as the latter ones might refer to well-known politicians. In order to recognize and tag mentions of well-known persons, we use we use the same entity recognition tagger used in the rest of paper~\cite{Ritter2011}. The rest of the algorithm remains unchanged.

We obtain the following results. In the month of November 2015 the first event retrieved by our algorithm is related to the declaration of François Hollande that France will close its borders in the aftermath of the November 13th attacks described by the following terms ``attacks'', ``France'', ``borders'', ``closes'', ``declares'', followed by an event about people being injured at protests calling for the resignation of South Korea's president (``Korea'', ``beaten'', ``happening'', ``people'', ``protesting''). In December 2015 most of the detected events are related to the presidential elections in the US (``bernie'', ``hillary'', ``\#demdebate'', ``war''), however, we find also a mention of the killing of peaceful protesters during a pro-Biafra protest (nigerian, \#ipob, navy, police, protesters, shooting, unarmed). In January 2016 the UN holds an emergency meeting after North Korea claims having done a nuclear test (North Korea, council, emergency, meeting, security, set, test), while in February 2016 Jeb Brush and Rand Paul suspend their presidential campaigns.  Another event detected in February is related to the Yemen civil war (Yemen, \#usakillyemenis, saudi-led, us-backed) and was triggered by a bombing at a cement factory close to the capital of Yemen, which resulted in the death of civilians. 

Those preliminary results show that our approach is robust and it has good potential in providing meaningful results for other classes of events. This will be investigated in the future.

==> cliques.tex <==
\section{Weighted quasi-cliques}

Let G be an undirected graph $G=(V(G),E(G))$, $w$ a weight function $w: E(G) \rightarrow \mathbb{R}^+$ and $\alpha$ a rational number $ \in [0,1]$. 

\noindent\textbf{Definition}
Let $H$ be a subgraph of $G$ such that:

\[\sum{w(e)}_{e \in E(H)} = w_{max}(H) \binom{|V(H)|}{2} \]

where $w_{max}(H) = \max_{e \in E(H)}(w(e)) $. We refer to $H$ as a weighted clique of $G$. Let $WC$ be the set of weighted cliques of $G$. 


To the best of our knowledge, this is the first time a weighted clique (or $\alpha$-quasi) is defined in such a way. Other definition are:

\textbf{put definitions}

By looking at the examples in Figure, we can notice that such definitions fail to differentiate between subgraphs. 

\bigskip
\noindent\textbf{Definition}
Let $H$ be a subgraph of $G$ such that:
\begin{equation}
\label{quasi}
\sum{w(e)}_{e \in E(H)} \geq \alpha w_{max}(H) \binom{|V(H)|}{2}
\end{equation}


where $w_{max}(H) = \max_{e \in E(H)}(w(e)) $. We refer to $H$ as a weighted $\alpha$-quasi-clique of $G$. Let $WQC$ be the set of weighted $\alpha$ quasi cliques of $G$. 

In the following we are going to focus on weighted $\alpha$-quasi-cliques of $G$, as cliques are a special case of quasi cliques. 

\bigskip
\noindent\textbf{Problem}
Given an undirected graph $G=(V(G),E(G))$, a weight function $w: E(G) \rightarrow \mathbb{R}^+$ and a rational number $\alpha \in [0,1]$, find a weighted $\alpha$-quasi-clique $H$ of $G$ such that:

\[\sum{w(e)}_{e \in E(H)} \geq  \sum{w(e)}_{e \in E(S)}\], $ \forall S \in WQC$. We refer to $H$ as the \textbf{maximum weighted $\alpha$-quasi clique}. 

Notice that all definitions and problems hold for an unweighted graph. 



\bigskip
\begin{theorem}
Every weighted $\alpha$-quasi clique $H$ of size $k$ contains at least one proper subgraph $H^{'}$ of size $k-1$ that is also a weighted $\alpha$-quasi clique. 
\end{theorem}

\begin{proof}
We can obtain this subgraph by removing from $H$ the node with minimum degree. The minimum degree of a node $v$ in $H$ such that $H$ is a weighted $\alpha$-quasi clique is 
\end{proof}
 

\bigskip
\noindent\textbf{Definition}
Let $H$ be weighted $\alpha$-quasi clique and $\forall v \in V(G) \setminus V(H)$:
\[\sum{w(e)}_{e \in E(H \cup v)} < \alpha w_{max}(H \cup v) \binom{|V(H)| + 1}{2},  \]
then $H$ as a \textbf{maximal weighted $\alpha$-quasi clique}.


\bigskip
\noindent\textbf{Problem}
Given an undirected graph $G=(V(G),E(G))$, a weight function $w: E(G) \rightarrow \mathbb{R}^+$ and a rational number $\alpha \in [0,1]$, find a maximal weighted $\alpha$-quasi-clique $H$ of $G$ such that:

\[ \frac{\sum{w(e)}_{e \in E(H)}}{|V(H)|}  \geq  \frac{\sum{w(e)}_{e \in E(S)}}{|V(S)|}\], $ \forall S \in WQC$. We refer to $H$ as the \textbf{maximum average weighted $\alpha$-quasi clique}.

\bigskip

==> preliminaries.tex <==


